Charge collection characterisation with the Transient Current Technique of the ams H35DEMO CMOS detector after proton irradiation

This paper reports on the characterisation with Transient Current Technique measurements of the charge collection and depletion depth of a radiation-hard high-voltage CMOS pixel sensor produced at ams AG. Several substrate resistivities were tested before and after proton irradiation with two different sources: the 24 GeV Proton Synchrotron at CERN and the 16.7 MeV Cyclotron at Bern Inselspital.

==> results.tex <==
\section{Results}
\label{sec:results}
